Goldman-Turaev formality from the Kontsevich integral

We present a new solution to the formality problem for the framed Goldman--Turaev Lie bialgebra, constructing Goldman-Turaev homomorphic expansions (formality isomorphisms) from the Kontsevich integral. Our proof uses a three dimensional derivation of the Goldman-Turaev Lie biaglebra arising from a low-degree Vassiliev quotient -- the {\em emergent} quotient -- of tangles in a thickened punctured disk, modulo a Conway skein relation. This is in contrast to Massuyeau's 2018 proof using braids. A feature of our approach is a general conceptual framework which is applied to prove the compatibility of the homomorphic expansion with both the Goldman bracket and the technically challenging Turaev cobracket.

==> KontsevichIntro.tex <==
\subsection{The Kontsevich Integral}\label{sec:KInt}
The Kontsevich Integral is the knot theoretic prototype of a {\em homomorphic expansion}. Homomorphic expansions (a.k.a. formality isomorphisms, universal finite type invariants) provide a connection between knot theory and quantum algebra/Lie theory.
Many detailed expositions on the Kontsevich Integral exist in the literature, we recommend \cite[Section 8]{CDM_2012}, or \cite{Kon, BN1, Da}. We briefly review the basics here from an algebraic perspective, which is outlined -- in a slightly different, finitely presentated case -- in \cite[Section 2]{WKO2}. 

Let $\calK$ denote the set of oriented knots in $\R^3$, and allow formal linear combinations of knots with coefficients in $\C$. There is a filtration on this infinite dimensional vector space called the Vassiliev filtration, which is defined in terms of resolutions of {\em double points.} Namely, a {\em double point} is defined to be the difference of an over and under crossing:
$$\dpcross = \pcross - \ncross.$$
A knot with $k$ double points is a signed sum of $2^k$ knots. See Figure \ref{fig:pumpkins} for an example.
The Vassiliev filtration is the decreasing filtration
$$\calK = \calK_0 \supseteq \calK_1 \supseteq \calK_2 \supseteq ...$$
where $\calK_i$ is linearly generated by knots with at least $i$ double points.

\begin{figure}
\centering
\begin{picture}(300,100)
\put(-30,0){\includegraphics[scale=.6]{doubleknotwithfourterms.pdf}}
\put(35,30){\Large{$=$}}
\put(110,30){\Large{$-$}}
\put(182,30){\Large{$-$}}
\put(255,30){\Large{$+$}}
\end{picture}
\caption{A knot with two double points written as a signed sum four knots.}
\label{fig:pumpkins}
\end{figure}

The degree completed associated graded space of $\calK$ with respect to the Vassiliev filtration is defined as
$$\calA:= \prod_{n \geq 0} \calK_n/\calK_{n+1}.$$
Since $\calA$ is a graded vector space, it lends itself naturally to recursive calculations and inductive arguments. %The key idea of Goussarov and Vassiliev was to study knots (the space $\calK$) via invariants which take values in $\calA$.
An {\em expansion} $Z$ is a filtered linear map of knots taking values in $\calA$, which retains as much information as possible. Rigorously, this means that the associated graded map of $Z$ is the identity map of $\calA$:
$$Z: \calK \to \calA \quad \text{such that} \quad \gr Z= id_\calA.$$ 
An expansion is {\em homomorphic} with respect to some operations (such as connected sum) if it also intertwines these operations  with their associated graded counterparts. This allows for a study of these operations via the associated graded space as well.

A crucial step towards making effective use of this machinery is to get a handle on the space $\calA$ in concrete terms: namely, $\calA$ has a combinatorial description as a space of {\em chord diagrams}. A chord diagram of degree $k$ on an oriented circle  is a perfect matching\footnote{A perfect matching on a set is a partitioning of the set by 2-element subsets.} on a set of $2k$ points arranged around the circle, up to orientation preserving diffeomorphism. The circle which supports the chord diagram is called the {\em skeleton}. In other words, a chord diagram on a circle is a combinatorial object consisting of $2k$ cyclically ordered points, partitioned into pairs. In diagrams, each pair is indicated by a {\em chord}, as in the left of Figure~\ref{fig:psionchord}. 


There is a natural map $\psi$ from chord diagrams with $i$ chords to $\calK_i/\calK_{i+1}$, as shown in Figure~\ref{fig:psionchord}. Namely, by contracting each chord into a double point, we obtain an $i$-singular knot. This is well-defined only up to crossing changes -- as crossings other than double points may appear -- however, the difference between the over/under choices for any additional crossing is in $\calK_{i+1}$.

\begin{figure}
\centering
\begin{picture}(200,60)
\put(-10,0){\includegraphics[scale=.7]{psiOnChordToKnot.pdf}}
\put(80,20){\Large{$\mapsto$}}
\put(84,30){{$\psi$}}
\end{picture}
\caption{Example of $\psi$ mapping a chord diagram to a singular knot where the right-hand side is viewed as an element of $\calK_3/\calK_{4}$.}
\label{fig:psionchord}
\end{figure}



It is not difficult to establish that $\psi$ is surjective, and that there are two relations in its kernel: the 4-Term (4T) and Framing Independence (FI) relations, shown in Figure~\ref{fig:4TFI}.   In fact, these two relations generate the kernel, and $\psi$ descends to an isomorphism on the quotient; this, however, is significantly harder to prove.

\begin{figure}[h]
\centering
\begin{picture}(300,70)
\put(-45,0){\includegraphics[scale=.7]{4TFI.pdf}}
\put(340,23){\Large{$0$}}
\put(322,33){\large{FI}}
\put(324,23){\Large{$=$}}
\put(220,23){\Large{$0$}}
\put(198,33){\large{4T}}
\put(200,23){\Large{$=$}}
\put(136,23){\Large{$-$}}
\put(70,23){\Large{$+$}}
\put(5,23){\Large{$+$}}
\put(-53,23){\Large{$-$}}
\end{picture}
\caption{The 4T and FI relations, understood as local relations: the strand(s) are part(s) of the skeleton circle, and the skeleton may support additional chords outside the picture shown, which are the same throughout all terms of the relation.}
\label{fig:4TFI}
\end{figure}

The key technique is to construct an expansion as in the following Lemma, \cite[Proposition 2.7]{WKO2}: 

\begin{lem}\cite{WKO2} \label{lem:assocgradyoga}
Let $\calK$ be a filtered space of formal linear combinations of knotted objects\footnote{``Knotted objects'' may mean knots, links, tangles, knotted graphs, etc, depending on context.}, and $\calA$ the associated graded space of $\calK$. Let $\calC$ be a ``candidate model'' for $\calA$: a graded linear space equipped with a surjective graded map $\psi: \calC \to \calA$. If there exists a filtered map $Z: \calK \to \calC$, such that $\psi \circ \gr Z = id_{\calA}$, then $\psi$ is an isomorphism and $Z$ is an expansion for $\calK$.


\[ \begin{tikzcd}
\calK \arrow{r}{Z} & \calC \arrow[dd,"\psi"] &&& \calA \arrow[r,"\gr Z"]\arrow[ddr,dashed, "\psi\circ \gr Z=id_{\calA}" left] & \calC \arrow[dd,"\psi"]\\
&&\text{ }\arrow[r,Mapsto, "\gr"] &\text{ }&&\\
& \calA&&&& \calA
\end{tikzcd}
\]

\end{lem}

In other words, once one finds a candidate model $\calC$ for $\calA$, finding an {\em expansion valued in} $\calC$ also implies that $\psi$ is an isomorphism.
In classical Vassiliev theory, $\calK$ is the space of oriented knots, $\calC$ is the space of chord diagrams, and a $\calC$-valued expansion is the Kontsevich integral \cite{Kon}.

For a detailed introduction to the Kontsevich integral we recommend \cite[Section 8]{CDM_2012}. The definition an explicit integral formula associated to a Morse representation of a knot or link in $\C \times \R$, as in Figure~\ref{fig:Kint}. 
\nsnote{Note from Dror: reconsider depth of discussion of $Z$}
\begin{definition}Let $K$ be an oriented link in $\R^3\cong \R_t\times \C$, where $t$ parametrises the vertical real dimension, and the embedding $K$ is Morse with respect to $t$: that is, critical points are cups or caps.
The unnormalised Kontsevich integral $Z'(K)$ of $K$ is defined as:
\begin{equation}\label{eq:Kint}
Z'(K):=\sum_{m=0}^{\infty} \thinspace
\mathop{\int\limits_{t_{min}<t_m<...<t_1<t_{max}}}_{t_i \thinspace non-critical} 
\sum_{P=\{(z_i,z_{i}')\}_i}
\frac{(-1)^{P_{\downarrow}}}{(2\pi i)^m}
\frakD_P \bigwedge_{i=1}^{m} \frac{dz_i-dz_i'}{z_i-z_i'}
.
\end{equation}
Here the values $t_{min}$ and $t_{max}$ denote the minimum and maximum heights of K, and each summand is an integral over an $m$-simplex determined by $t_m<\cdots< t_1$.
The summation is over choices $P$ of ``pairings'' of two points on the knot of height $t_i$, each of which, when projected to the plane at $t=0$, yields a complex pair $(z_i,z_i')$.
We denote by $\frakD_P$ the chord diagram given by interpreting the $m$ pairings $(z_i,z_i')$ as chords, as shown in Figure~\ref{fig:Kint}. 
Finally, $P_\downarrow$ is the number of points in $P$ where $(t_i,z_i)$ or $(t_i,z_i')$ is on a $t$-descending arc in $K$.
\end{definition}

\begin{figure}
\centering
\begin{picture}(150,130)
\put(-55,0){\includegraphics[scale=.47]{kontsevichknot.pdf}}
\put(-2,7){$z_1$}
\put(13,7){$z_1'$}
\put(-62,33){$t_1$}
\put(-62,62){$t_2$}
\put(-62,80){$t_3$}
\put(-62,105){$t_4$}
\put(200,90){$1$}
\put(175,98){$2$}
\put(185,55){$3$}
\put(177,41){$4$}
\put(140,25){$\frakD_P$}
\end{picture}
\caption{The Kontsevich Integral is computed from a Morse embedding of the knot}\label{fig:Kint}
\end{figure}

Kontsevich's famous result \cite{Kon} is that $Z(K):=\frac{Z'(K)}{Z'(\hump)^{c/2}}$ is an invariant of unframed links, where $c$ denotes the number of critical points -- minima and maxima -- in the Morse embedding of $K$. The Kontsevich integral takes values in the space of chord diagrams (for links, with chords on multiple circles) modulo the 4T and FI relations. The Kontsevich integral $Z$ satisfies $\psi \circ \gr Z = id_{\calC}$. Therefore, $\psi$ is an isomorphism, and $Z$ is an expansion for unframed links. In light of this, we do not distinguish between $\calC$ and $\calA$, and use $\calA$ to mean  In addition, $Z$ has a number of good properties, for example, it is homomorphic with respect to knot connected sum. 

